AutoDDG: Automated Dataset Description Generation using Large Language Models

The proliferation of datasets across open data portals and enterprise data lakes presents an opportunity for deriving data-driven insights. Widely-used dataset search systems rely on keyword search over dataset metadata, including descriptions, to support discovery. Therefore, when these descriptions are incomplete, missing, or inconsistent with dataset contents, findability is severely compromised. To improve findability, we introduce AutoDDG, a framework that automatically generates descriptions of tabular data. By adopting a data-driven approach to summarize dataset contents and leveraging large language models (LLMs) to enrich summaries with semantic information and produce human-readable text, AutoDDG derives descriptions that are comprehensive, accurate, readable, and concise. A critical challenge in this problem is evaluating the effectiveness of description generation methods and assessing the quality of the generated descriptions. We propose a comprehensive evaluation methodology that combines retrieval, reference-based, and reference-free assessment, with human validation. Our experimental results using new benchmarks demonstrate that AutoDDG generates high-quality, accurate descriptions at scale, significantly improving dataset retrieval performance across diverse use cases. AutoDDG is publicly available at https://github.com/VIDA-NYU/AutoDDG.

==> tables/prompt_faithfulness.tex <==
\begin{table*}
    \small
    \centering
    \begin{tabular}{p{14cm}}
    \toprule
    \textbf{Dataset Description Faithfulness Evaluation Prompt} \\
    \midrule
    \textcolor{teal}{\textbf{Task Description:}} \\
    Your task is to evaluate whether the given dataset description faithfully represents the facts from the provided dataset sample, dataset profile, and semantic profile. For each sentence in the description, verify whether it accurately reflects the information from the inputs. Carefully check step-by-step for every sentence to determine if it is true or false. Use Example 1 as a reference and respond to Example 2. \\
    \\
    \textcolor{teal}{\textbf{Example 1}} \\
    \textbf{Dataset Sample:} \\
    \texttt{Time Stamp, Average Wind Speed, Standard Deviation, Average Wind Direction} \\
    \texttt{7/22/2003 1:40, 1.8, 1.66, 315} \\
    \texttt{6/18/2003 10:50, 6.0, 1.44, 225} \\
    \\
    \textbf{Dataset Profile:} \\
    - **Time Stamp:** Data is of type text, 13,576 unique values, semantic type: datetime. \\
    - **Average Wind Speed:** Data is of type float, range: 0 to 30.2. \\
    - **Standard Deviation:** Data is of type float, range: 0 to 3.05. \\
    - **Average Wind Direction:** Data is of type integer, 16 unique values, range: 0 to 338.0. \\
    \\
    \textbf{Semantic Profile:} \\
    - **Time Stamp:** Represents temporal entity, resolution: Hour. \\
    - **Average Wind Speed:** Represents measurement, domain: climate, function: measurement. \\
    - **Standard Deviation:** Represents statistical measure, domain: general, function: measurement. \\
    - **Average Wind Direction:** Represents measurement, domain: climate, function: measurement. \\
    \\
    \textbf{Data Topic:} Wind Speed Data \\
    \\
    \textbf{Generated Description:} \\
    "This dataset contains 13,576 hourly records of wind speed and direction, with wind speed ranging from 0 to 30.2 m/s and wind direction values spanning from 0 to 360°. It includes detailed hourly timestamps as temporal entities, with wind speed and direction categorized as climate measurements. This dataset is useful for renewable energy planning, meteorological research, and understanding wind patterns." \\
    \\
    \textbf{Evaluation:} \\
    - **(Sentence 1):** "This dataset contains 13,576 hourly records of wind speed and direction, with wind speed ranging from 0 to 30.2 m/s and wind direction values spanning from 0 to 360°." \\
      **Explanation:** The dataset profile specifies 13,576 records, the correct wind speed range (0–30.2 m/s), and the correct timestamp type. However, the wind direction range is incorrectly stated as 0–360° instead of 0–338°. \\
      **Verification:** F \\
    - **(Sentence 2):** "It includes detailed hourly timestamps as temporal entities, with wind speed and direction categorized as climate measurements." \\
      **Explanation:** The semantic profile confirms that the timestamps are temporal entities, and wind speed and direction are categorized as climate measurements. \\
      **Verification:** T \\
    - **(Sentence 3):** "This dataset is useful for renewable energy planning, meteorological research, and understanding wind patterns." \\
      **Explanation:** These applications are reasonable inferences based on the dataset's focus on wind speed and direction. \\
      **Verification:** T \\
    \\
    \textcolor{teal}{\textbf{Example 2}} \\
    \textbf{Dataset Sample:} \texttt{\{dataset\_sample\}} \\
    \textbf{Dataset Profile:} \texttt{\{dataset\_profile\}} \\
    \textbf{Semantic Profile:} \texttt{\{semantic\_profile\}} \\
    \textbf{Data Topic:} \texttt{\{data\_topic\}} \\
    \textbf{Generated Description:} \texttt{\{dataset\_description\}} \\
    \\
    \textbf{Evaluation:} \\
    (Sentence 1): \texttt{\{\{sent1\}\}} \\
    (Explanation): \texttt{\{\{explanation\}\}} \\
    (Verification): T/F \\
    ... \\
    (Sentence n): \texttt{\{\{sent n\}\}} \\
    (Explanation): \texttt{\{\{explanation\}\}} \\
    (Verification): T/F \\
    \bottomrule
    \end{tabular}
    \caption{Prompt for evaluating dataset description faithfulness based on dataset sample, profile, and semantic profile.}
    \label{tab:faithfulness_evaluation}
\end{table*}


% \begin{table*}
%     \small
%     \centering
%     \begin{tabular}{p{14cm}}
%     \toprule
%     \textbf{Dataset Description Faithfulness Evaluation Prompt} \\
%     \midrule
%     \textcolor{teal}{\textbf{Task Description:}} \\
%     Your task is to evaluate whether the given dataset description faithfully represents the facts from the provided dataset sample, dataset profile, and semantic profile. For each sentence in the description, verify whether it accurately reflects the information from the inputs. Carefully check step-by-step for every sentence to determine if it is true or false. Use Example 1 as a reference and respond to Example 2. \\
%     \\
%     \textcolor{teal}{\textbf{Scoring Guidelines:}} \\
%     - **High Score (8-10):** All claims are explicitly supported by the dataset inputs or are reasonable inferences that logically follow from the data. Broader usage or applications are acceptable if plausible. \\
%     - **Moderate Score (5-7):** The description is mostly faithful but includes some loosely supported or slightly overstated claims. \\
%     - **Low Score (1-4):** Several claims are unsupported, speculative, or deviate significantly from the dataset inputs. \\
%     \\
%     \textcolor{teal}{\textbf{Example 1}} \\
%     \textbf{Dataset Sample:} \\
%     \texttt{Time Stamp, Average Wind Speed, Standard Deviation, Average Wind Direction} \\
%     \texttt{7/22/2003 1:40, 1.8, 1.66, 315} \\
%     \texttt{6/18/2003 10:50, 6.0, 1.44, 225} \\
%     \\
%     \textbf{Dataset Profile:} \\
%     - **Time Stamp:** Data type: text, 13,576 unique values, semantic type: datetime. \\
%     - **Average Wind Speed:** Data type: float, range: 0 to 30.2. \\
%     - **Standard Deviation:** Data type: float, range: 0 to 3.05. \\
%     - **Average Wind Direction:** Data type: integer, 16 unique values, range: 0 to 338.0. \\
%     \\
%     \textbf{Semantic Profile:} \\
%     - **Time Stamp:** Represents temporal entity, resolution: Hour. \\
%     - **Average Wind Speed:** Represents measurement, domain: climate, function: measurement. \\
%     - **Standard Deviation:** Represents statistical measure, domain: general, function: measurement. \\
%     - **Average Wind Direction:** Represents measurement, domain: climate, function: measurement. \\
%     \\
%     \textbf{Data Topic:} Wind Speed Data \\
%     \\
%     \textbf{Generated Description:} \\
%     "This dataset contains 13,576 hourly records of wind speed and direction, with wind speed ranging from 0 to 30.2 m/s and wind direction values spanning from 0 to 338°. It includes detailed hourly timestamps as temporal entities, with wind speed and direction categorized as climate measurements. This dataset is useful for renewable energy planning, meteorological research, and understanding wind patterns." \\
%     \\
%     \textbf{Evaluation:} \\
%     - **Faithfulness Score:** \textbf{8} \\
%     - **Explanation:** Most claims in the description are supported by the dataset profile and semantic profile. Statements about "predicting weather changes" and "renewable energy policies" are reasonable inferences based on the dataset's focus on wind speed and direction. However, "advancements in technology for wind energy generation" is speculative and reduces the score slightly. \\
%     \\
%     \textcolor{teal}{\textbf{Evaluation Task:}} \\
%     After reviewing the example above, evaluate the dataset description using the provided sample, profile, and semantic profile. Provide a detailed explanation for your rating. \\
%     \\
%     \textbf{Dataset Sample:} \texttt{\{dataset\_sample\}} \\
%     \textbf{Dataset Profile:} \texttt{\{dataset\_profile\}} \\
%     \textbf{Semantic Profile:} \texttt{\{semantic\_profile\}} \\
%     \textbf{Data Topic:} \texttt{\{data\_topic\}} \\
%     \textbf{Generated Description:} \texttt{\{dataset\_description\}} \\
%     \\
%     \textbf{Evaluation:} \\
%     - **Faithfulness Score (score only):** \_\_ \\
%     - **Explanation (in sentences):** \_\_\_\_ \\
%     \bottomrule
%     \end{tabular}
%     \caption{Prompt for evaluating dataset description faithfulness based on dataset sample, profile, and semantic profile.}
%     \label{tab:faithfulness_evaluation}
% \end{table*}

